Exploring the Potentials and Challenges of Using Large Language Models for the Analysis of Transcriptional Regulation of Long Non-coding RNAs

Research on long non-coding RNAs (lncRNAs) has garnered significant attention due to their critical roles in gene regulation and disease mechanisms. However, the complexity and diversity of lncRNA sequences, along with the limited knowledge of their functional mechanisms and the regulation of their expressions, pose significant challenges to lncRNA studies. Given the tremendous success of large language models (LLMs) in capturing complex dependencies in sequential data, this study aims to systematically explore the potential and limitations of LLMs in the sequence analysis related to the transcriptional regulation of lncRNA genes. Our extensive experiments demonstrated promising performance of fine-tuned genome foundation models on progressively complex tasks. Furthermore, we conducted an insightful analysis of the critical impact of task complexity, model selection, data quality, and biological interpretability for the studies of the regulation of lncRNA gene expression.

==> section/conclusion.tex <==

\section{Conclusion}
\label{sec:conclusion}
\begin{comment}
\begin{itemize}
    \item Summarize the major findings. 
    \item Highlight the contributions. 
    \item Future research directions 
\end{itemize}
\end{comment}

In this study, we studied the application of large language models (LLMs) to non-coding RNA (ncRNA) sequence analysis. We evaluated how well LLMs can capture complex sequence patterns and contribute to ncRNA studies by fine-tuning pre-trained foundation models, DNABERT, DNABERT-2, and the Nucleotide Transformer. 

The experiment results show that the LLMs are effective in multiple tasks, including biological and artificial sequence classification, promoter sequence detection, and gene expression classification. These results indicate that the LLMs can effectively capture complex sequence patterns and dependencies, offering significant advantages in genomic research. Additionally, the attention mechanisms used in these models enables us to identify which sequence regions are most important for predictions. This can potentially provide valuable biological insights into the regulatory mechanisms of ncRNAs and other cellular processes. 

One critical findings this study is the impact of data quality on model performance. We found that the biological and artificial sequence classification dataset was mistakenly used for promoter sequence detection purposes in DNABERT2, which simplified the task and made it less challenging. One evidence is that LLMs shows better performance on biological and artificial sequences than classification of promoter and biological but non-promoter sequences. The misuse of data can lead to over-optimistic model performance, misleading biological insights and wrong conclusions.
This finding highlights the importance of well defined, biologically meaningful datasets in machine learning applications, and rigorous data validation and task design in genomic studies. As for ncRNA analysis, this finding suggests that future efforts should prioritize improving dataset quality to better capture the complexity of ncRNA regulation and function.

Another finding is that traditional machine learning methods, logistic regression with n-gram TF-IDF features, achieved similar results to LLMs in certain tasks, especially those tasks with simpler datasets. This finding raises an important question, when the complexity of LLMs is truly needed? In some tasks, simpler models may be sufficient to provide comparable results with lower computational costs. This indicates that, for ncRNA analysis, not all tasks require the advanced modeling capabilities of LLMs. Simple traditional machine learning methods can provide more efficient and interpretable solutions at low cost. LLMs are more suitable for tasks that require deep contextual understanding, such as predicting complex regulatory motifs or interactions.

These findings also show the importance of integrating domain knowledge into LLM training and fine-tuning processes. As LLMs become more popular in ncRNA analysis, it is necessary to check the data quality and task design to ensure that these powerful models provide accurate and useful insights. By incorporating biological insights into model development and task design, we can guide LLMs to further improving both performance and interpretability. 


==> section/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

% \xr{I am not sure whether this is the writing style of this domain. I personally feel it probably better to merge these detailed analysis into each corresponding section in the experiments. Otherwise it looks far away from the results, and it may look quite disconnected (the reader needs to go back to carefully find the evidence). If there much be a section about discussion, some high-level discussion is probably better}

\begin{comment}

\subsection{Promoter sequence classification using LLMs}

Promoter sequences are critical regions that regulate transcription and play a critical role in gene expression. Identifying promoter sequences and their associated functional motifs is important to understand regulatory mechanisms, conduct disease analysis, and advance medical research. 

The quality of the data used in machine learning tasks significantly influences the model performance. In our study, we explored three distinct datasets to approximate different data quality and biological representations.

The first dataset derived from the GUE datasets was originally proposed for promoter and non-promoter sequence classification task. Due to inappropriate generation of negative samples, where positive sequences were reshuffled to create negative samples, the dataset reduced to biological and artificial sequence classification task. This is a easier task than the promoter and non-promoter sequence classification. 

The results show that the three foundation models consistently perform better in biological and artificial sequence classification tasks than the other two tasks, promoter sequence classification and promoter sequence classification of coding and noncoding genes, which confirmed that the dataset derived from the GUE dataset is a reduced task to biological and artificial sequence classification. 

We regenerate the promoter seqeunce and non-promoter sequence by reuse positive samples from GUE dataset and generating negative samples by random sampling from human genome outside of the promoter regions. This approach ensures that the negative samples contains biological context, representing a more realistic and challenging classification task. 
The slightly lower performance of three foundation models shows that this task represents the real complexity of promoter sequence idenfitication task. 

The coding and non-coding gene classification is a known difficult task. The low performance in the classification of promoter sequences of coding and non-coding genes reflects the complexity of this task. This indicates that the information provided by the promoter sequences is limited. Even the LLMs cannot identify gene type simply through promoter sequences. This task requires additional information and more sophisticated modeling techniques. 

These results show fine-tuned LLMs are effective tools for sequence analysis, such as promoter sequence classification, providing valuable insights into their regulatory functions. The variability in performance in three different tasks indicates that the data quality and biological meaning of the data set for model tuning play an important role in achieving the accurate classification results. 


\subsection{Comparing LLMs with Simpler Models}

The experiment results show that, despite advanced model architectures and extensive pre-training, LLMs didn't consistently outperform the simpler model in the experiemnts.  Simple model, n-gram logistic regression, already achieves robust performance on promoter sequence classification tasks. This finding raises important questions about the necessity and efficiency of using LLMs in biological sequence analysis. 

One possible reason for this problem is the nature of the task and the data. Promoter sequences may not require the deep contextual understanding that LLMs provide. Simple models leveraging certain sequence patterns effectively captured by n-grams and can perform well on the promoter sequence classification task. 

This observation suggests that LLMs may not always offer a significant advantage for all genetic analysis tasks. The analysis tasks that benefit from the advantage of LLMs are more complex tasks that requires more contextual information. 
To maximize the power of LLMs, the following strategies could be considered. LLMs should be fine-tuned on tasks with clear definition on high-quality and curated dataset that accurately represent the biological task of interest; integrating domain knowledge into the training process to enhance the performance of LLMs. This could involve embedding additional information into the model. 


\subsection{Biological insights in gene expression regularization}

Despite certain limitations, LLMs show unique insights in genomic sequence analysis. We perform a promoter sequence classification of high and low expression genes. This task serves as a proxy for understanding the regulatory mechanisms of coding and non-coding genes. This task shows better performance than the coding and non-coding gene promoter sequence classification task. This indicates that the promoter region plays an critical role in gene expression regulation, which is consistent with known publications.

We compared the model performance on promoter regions with different length, ranging from 300bp, 500bp, 1000bp, and 2000bp. The results indicate that 300bp promoter sequences produces better model performance compared to longer sequences 2000bp. This result provides important insights in the regularization functional region. This is likely because shorter sequences contain more specific regulatory elements that are easier for models to capture. As sequence length increases, the complexity and noise also increase, diluting the signal that models can learn from. Importantly, DNABERT (3-mer) performs best on 300bp sequences, while DNABERT-2 performs best on 2000bp sequences. This indicates that different models have different capacity to capture long-distance dependencies. This suggests that the selection of model should base on the specific length and complexity of the dataset.

To gain further insights into the critical regions that regulates gene expression and critical for promoter sequence classification, we conducted the feature importance analysis using the attention scores from the LLMs. 
\end{comment}


\begin{comment}
    

\begin{itemize}
    \item Dataset quality and biological meaning of the dataset influence model performance. \\
    Although the DNABERT2 article claimed that the dataset was used for classification of promoter and non promoter sequences. However, due to inappropriate negative sample generation and reshuffle of positive samples, the data set was reduced to a classification of biological and nonbiological data sets. \\
    The results show that this task is much easier than the promoter sequence classification task. Similar issues were observed in transcription binding site identification studies
    \item By comparing the performance of LLM and simple linear model, n-gram logistic regression, the result shows that these two models achieves similar performance on promoter sequence classfication task. The use of LLM may or may not result in advanced performance in biological tasks. Possible reasons why LLM may not outperform simple models, how to maximize the power of LLM. 
    \item Though there is limitation, LLM has its potential. We analyze the classification of promoter sequences of high- and low-expression genes. The results show consistency with known publications. By addressing the problem of data quality, with comprehensive experiment design and biological experimental validation, the LLM can be a powerful tool to boost biological studies. 
\end{itemize}
\end{comment}

This study explored the application of large language models (LLMs) in non-coding RNA (ncRNA) sequence analysis across various tasks, comparing their performance to traditional machine learning methods such as logistic regression. Our findings demonstrate that while LLMs excel in complex tasks, simpler models can still perform competitively in less challenging scenarios. Below, we discuss the key insights from our results, including the implications for data quality, task complexity, and model selection in future research.

LLMs such as DNABERT and DNABERT-2 outperformed traditional models in tasks like promoter sequence classification and gene expression prediction. The feature importance analysis revealed that the first 80bp of promoter sequences had the most significant impact on gene expression prediction, emphasizing the importance of the proximal promoter region in transcription regulation. This aligns with existing biological knowledge, where key regulatory elements are concentrated near the transcription start site (TSS). These findings suggest that LLMs, with their ability to capture long-range dependencies and complex sequence features, are particularly useful for uncovering regulatory mechanisms in genomic data. 
However, our results also show that simpler models, such as logistic regression, remain competitive in less complex tasks. For example, in the biological versus artificial sequence classification task, logistic regression achieved an MCC close to that of LLMs. This highlights that in scenarios where task complexity is low, simpler models can offer similar accuracy with significantly reduced computational cost. Therefore, selecting a model should depend on the complexity of the task at hand—LLMs are best reserved for tasks where deep contextual understanding is required, while simpler models are more efficient for straightforward classification problems.

Data quality emerged as a crucial determinant of model performance. In the biological versus artificial sequence classification task, artificially generated data inflated model performance, highlighting the need for well-curated, biologically meaningful datasets. Conversely, the coding versus non-coding gene promoter classification task proved more challenging for all models, reflecting the difficulty of distinguishing between these promoter types based solely on sequence data. This underscores the importance of using high-quality, task-specific data when applying LLMs in biological research.

The impact of promoter sequence length on model performance was another key finding. Models performed best with shorter promoter sequences (300bp), and performance declined as the sequence length increased, likely due to added complexity and noise. Shorter sequences tend to contain more concentrated regulatory elements, making it easier for models to capture relevant features. Thus, selecting appropriate sequence lengths is critical for optimizing model accuracy in future research.

The attention-based feature importance analysis also provided valuable biological insights, revealing that LLMs can highlight key regulatory regions within sequences. This capability enhances model interpretability and supports the discovery of novel regulatory motifs. Integrating domain knowledge into model training can further improve the accuracy and interpretability of these models, making them more applicable to real-world biological problems.

==> section/experiment.tex <==
\section{Results}
\label{sec:results}


% \xr{here, I think we might need to provide some high-level description of how and why we design these prediction tasks, in particular, why they are useful or critical for non-coding RNA analysis. Currently, it is a bit unclear how these studies are related to ncRNA analysis}


% \xr{It seems the following sections are organized by the methods, first LLM and then simple models. I think this organization is not very naturally. Would it be better or clearer if we organized the sections according the prediction tasks? It may be also easier to provide some analysis or discussion for each prediction task.}

This section presents the findings from the experiments, evaluating the performance of large language models (LLMs) in ncRNA analysis related tasks. We fine-tuned DNABERT, DNABERT-2, and the Nucleotide Transformer, and compared their performance across multiple tasks and against a traditional logistic regression model. The results are organized according to the specific tasks we tested.





\begin{comment}
\begin{itemize}
    \item Fine-tune DNABERT, DNABERT2, and Nucleotide transformer models. Description of foundation models, list parameters and computational costs. 
    \item Task description: 1. biological and non-biological sequence classification, 2. promoter and non-promoter sequence classification, 3. coding and non-coding promoter sequence classification. 
    \item Logistic regression model training for promoter sequence classification. 
\end{itemize}



\subsection{Measurements}
MCC, F1 score, accuracy, precision, recall \\ 
DNABERT-vis analysis \\
Transformer-interpret description \\ 

\xr{we can have three subsections. In each subsection, we can describe the dataset, experimental setting, results, and analyses}
\end{comment}

\textbf{Biological and artificial sequence classification} We evaluated the performance of fine-tuned foundation models on the biological and artificial sequence classification task. This task is less challenging because of the significant difference between real biological sequences and reshuffled artificial sequences. As shown in Table 1, DNABERT (3-mer) achieved the highest Mathews correlation coefficient (MCC) of 93.8, followed closely by DNABERT-2 (92.59) and Nucleotide Transformer (89.89). The logistic regression model also performed well on this task, achieving an MCC of 86.68. This shows that for this simple task, traditional machine learning method is almost as effective as the advanced LLMs with much less model complexity and computational cost. 

\textbf{Promoter and non-promoter sequence classification} The second task focused on distinguishing between promoter and non-promoter sequences. This task has a higher level of complexity. In this task, DNABERT (3-mer) once again outperformed the other models, achieving an MCC of 83.41. The Nucleotide Transformer showed a similar performance with an MCC of 83.23, while DNABERT-2 achieved 80.58 and the logsitic regression model achieved 75.03. 
Compared to the biological and artificial classification task, the performance of all models decreased. The detection of promoter regions shows more challenge to computational methods. The logistic regression model also experienced a significant performance drop, shows the limits of simpler models in handling complex tasks. 

\textbf{Coding and non-coding gene promoter classification} 

The most challenging task was the classification of coding and non-coding gene promoter sequences. As expected, the performance of all models was significantly lower in this task. DNABERT-2 achieved the highest MCC of 41.93, slightly outperforming DNABERT (3-mer) with 41.55. The Nucleotide Transformer performed the worst, with an MCC of 35.72. Surprisingly, the logistic regression model achieved MCC of 37.10, better than the Nucleotide Transformer on this task. This result indicates that the LLMs did not fully capture the contextual information to distinguish coding and non-coding gene promoters. The simple models can be competitive in certain tasks.

% The results show that the biological and artificial sequence classification task has the overall highest model performance. Then the promoter sequence and non-promoter sequence classification task. The promoter sequence classification task of coding and non-coding genes has the overall worst performance. 
% Different foundation models have similar model performance on three tasks. The DNABERT (3-mer) achieves the best performance on biological sequence classification and promoter sequence classification. The DNABERT-2 performs the best on promoter sequence classifcation of non-coding genes. 

\begin{table}[h]
\vspace{-0.2in}
    \centering
    \caption{Fine-tuned model performance on three tasks measured by atthews correlation coefficient (MCC), biological or non biological sequence classification, promoter or non promoter sequences classification, and promoter sequence of coding and non coding gene classification.}
    \begin{tabular}{lccc}
        \hline
        Model & Biological & Promoter & Non-coding \\
        \hline
        DNABERT (3-mer)&93.8&83.41&41.55\\
        NT-500M-human&89.89&83.23&35.72\\
        DNABERT-2&92.59&80.58&41.93\\
        LG&86.68 &75.03 &37.10\\
        \hline
    \end{tabular}
    \label{tab:three_tasks}
    \vspace{-0.2in}
\end{table}



\begin{comment}
\xr{we need to describe how we set up and tune the setting and hyperparameters}
\end{comment}

% \subsection{Simple model on promoter and non-promoter sequence classification}
% We train simple logistic regression models on three datasets used in a previous experiment, the biological and artificial sequence data set, the promoter and non-promoter sequence data set, and the promoter sequence data set of the coding and non-coding genes. 


% LR achieved slightly worse results on three tasks compared with fine-tuned LLM models. 86.68 MCC on biological sequence classification, 75.03 on promoter sequence classification, and 37.10 on non-coding promoter sequence classification. One thing to be notice is that the LR model achieves better performance than NT-500M-human model on non-coding promoter sequence classification task. This indicate that there is no guarantee for the LLM to achieve advanced model performance on all tasks. 

% \begin{table}[h]
% \vspace{-0.2in}
%     \centering
%     \caption{Logistic regression model performance on three tasks.}
%     \begin{tabular}{lccc}
%         \hline
%         Task & MCC & Accuracy & F1 Score \\
%         \hline
%         Biological & 86.68 & 93.33 & 93.33 \\
%         Promoter & 75.03 & 87.49 & 87.72 \\
%         Non-coding & 37.10 & 69.64 & 62.50 \\
%         \hline
%     \end{tabular}
%     \label{tab:performance_metrics}
%     \vspace{-0.2in}
% \end{table}

\textbf{Promoter sequence classification of high and low expressed genes} 
This task is designed to explore the regulatory mechanisms associated with gene expression. As shown in Table \ref{tab:high_low_exp}, DNABERT (3-mer) achieved the best performance with an MCC of 73.48, followed by Nucleotide Transformer 70.10 and DNABERT-2 67.78. These results show that LLMs are more effective on tasks that need deeper contextual understanding, such as the complex relationships between promoter sequences and gene expression levels.

\begin{table}[h]
\vspace{-0.2in}
\centering
\caption{Model performance on promoter sequence (300bp) classification of high and low expression genes}
\begin{tabular}{lcccc}
    \hline
    Model & MCC & Accuracy & F1 Score \\
    \hline
    DNABERT (3-mer) & 73.48 & 87.95 & 86.61 \\
    NT-500M-human & 70.10 & 86.59 & 84.99 \\
    DNABERT-2 & 67.78 & 86.22 & 83.68 \\
    \hline
\end{tabular}
\vspace{-0.1in}
\label{tab:high_low_exp}
\end{table}


To evaluate the impact of sequence length on model performance, we also set an experiment on promoter sequence classification of high and low expressed genes with different lengths of promoter sequences: 300bp, 500bp, 1000bp, and 2000bp. 
The results, shown in Table \ref{tab:model_performance}, indicate that shorter promoter sequences (300bp) produced better performance across all models. As the sequence length increased, the performance decreased. DNABERT (3-mer) achieved the best results with an MCC of 73.48 on the 300bp sequences, while DNABERT-2 performed better on longer sequences (2000bp) with an MCC of 45.73. These findings suggest that shorter sequences already cover specific regulatory regions, thus it is easier for models to capture. Longer sequences introduce additional complexity and noise. 

\begin{table}[h]
    \centering
    \caption{Comparison of model performance across different promoter sequence lengths on promoter sequence classification of high and low expression genes}
    \begin{tabular}{lcccc}
        \hline
        Model & 300bp & 500bp & 1000bp & 2000bp \\
        \hline
        DNABERT (3-mer) & 73.48 & 67.69 & 49.72 & 37.46 \\
        NT-500M-human & 70.10 & 65.73 & 51.90 & 34.26 \\
        DNABERT-2 & 67.78 & 69.11 & 46.48 & 45.73 \\
        \hline
    \end{tabular}
    \label{tab:model_performance}
\end{table}

\textbf{Parameter sensitivity and model analysis}
To further investigate model behavior, we conducted a parameter sensitivity study on promoter sequence detection task with DNABERT using different k-mer sizes (3-mer, 4-mer, 5-mer, and 6-mer). As shown in Table \ref{tab:dnabert_kmer}, the performance of DNABERT remained stable across different k-mer sizes. The 3-mer DNABERT shows the best results. This suggests that DNABERT is relatively robust to the choice of k-mer on ncRNA sequence classification tasks.

\begin{table}[h]
\vspace{-0.2in}
    \centering
    \caption{Parameter sensitivity study on DNABERT with different k-mer.}
    \begin{tabular}{lccc}
        \hline
        Model & MCC & Accuracy & F1 Score \\
        \hline
        DNABERT (3-mer) & 83.41 & 92.67 & 92.67 \\
        DNABERT (4-mer) & 83.06 & 92.52 & 92.52 \\
        DNABERT (5-mer) & 82.96 & 91.44 & 91.44 \\
        DNABERT (6-mer) & 83.13 & 92.56 & 92.56 \\
        \hline
    \end{tabular}
    \label{tab:dnabert_kmer}
    \vspace{-0.2in}
\end{table}

% \textbf{Insights into gene expression by promoter sequence classification of high and low expression genes}

% The classification of promoter sequences of coding and non-coding genes is a challenging task because of the complex nature of promoter regions and the subtle differences between coding and non-coding gene promoters. 
% To address this problem, we built a dataset to approximate this task by focusing on the classification of promoter sequences of high and low expressed genes.
% Gene expression levels represent activity and serve as an important indicator of gene functions. We can indirectly assess the function of non-coding RNA by gaining insights into the regularization mechanism. The rationale behind this idea is supported by statistical analysis, as shown in Table~\ref{tab:gene_stats} and Fig~\ref{fig:gene_expression}. The average expression level of non-coding genes is significantly lower than the coding genes. By split genes by their expression, majority of high expressed genes are coding genes, and non-coding genes are mainly low expressed and mid expressed genes. These observations indicate that non-coding genes are in general low expression genes. By predict gene expression level, we can indirectly predict the gene type with relatively high accuracy.  



\begin{comment}
\subsubsection{Model fine-tuning}
We conducted the same fine-tuning on three foundation models, DNABERT (3-mer), NT-500M-human, and DNABERT2. The MCC of three models shows comparable results, where the best model is DNABERT (3-mer), then NT-500M-human. DNABERT2, through is the most recent model shows the worst model performance. We did not further tune the model parameters, all hyperparameters are obtained from DNABERT2\cite{zhou2023dnabert2}, thus there is still room to improve. 
\end{comment}


% For the promoter sequence (300bp) classification task of high and low expression genes, the model performance is better than promoter sequence classification of coding and non-coding genes, and worse than the promoter and non-promoter sequence classification. This result indicates that the classification of promoter sequence of high and low expression genes is a relatively easier task than the coding and non-coding gene classification task, but more difficult than the promoter sequence classification task. The DNABERT (3-mer) shows the best performance on this task, achieves 73.48 MCC. The DNABERT-2 shows worst performance, 67.78 MCC. 

% We compared the performance of the model on the dataset with different promoter sequence length. The result shows best model performance on 300bp promoter sequences. As sequence increase, the model performance decrease. As the promoter sequence increased to 2000bp, the model performance is about half as the model performance of 300bp. 

% An interesting observation is that on 300bp, DNABERT (3-mer) performs the best. On 2000bp, DNABERT-2 shows the best performance, indicating different model ability on capture the information hide in long-distance dependency. 



\textbf{Feature importance analysis}

We conducted a feature importance analysis through the attention mechanisms of the LLMs. 
For the gene expression prediction task, the feature importnace analysis results indicates that the the initial 80bp upstream of the transcription start site (TSS), contributes the most to the prediction of gene expression levels. This 80bp region likely contains key regulatory elements that strongly influence gene expression. 
This finding aligns with existing biological knowledge and our experiments on various promoter sequence length that proximal promoter regions often contain critical binding sites for transcription factors that regulate gene expression.
% These results show the importance of integrating attention-based model insights to pinpoint biologically relevant sequence regions, which can aid in the discovery of functional motifs and the understanding of gene regulation mechanisms.



\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/high_expression_feature_importance_layer7_reverse.png}
        \caption{High expression genes.}
        \label{fig:high_exp_feat_ipt}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/low_expression_feature_importance_layer7_reverse.png}
        \caption{Low expression genes.}
        \label{fig:low_exp_feat_ipt}
    \end{subfigure}
    \caption{Feature importance distribution of promoter sequences of high and low expression genes.}
    \label{fig:exp_feat_ipt}
\end{figure}


\begin{comment}
\begin{itemize}
    \item Compare the results of three tasks. 
    \item Compare LLM and logistic regression results. 
    \item Promoter sequence classfication of high and low expression genes, DNABERT-vis/transformer-interpret visualization results, overlap with known publications. \todo[inline,color=yellow]{1. run DNABERT-vis; 2. summarize important features/regions, check previous biological studies}
\end{itemize}
\end{comment}

==> section/intro.tex <==

\section{Introduction}
\label{sec:introduction}
\begin{comment}
\begin{itemize}
    \item Introduction of non-coding RNA analysis. \\
    Definition and biological function of ncRNA. \\
    Challenges of non-coding RNA analysis, highly complexe and diverse sequences, noisy data with limit knowledge and high quality annotation, challenging in experimental validation.  \\
    Summarize the latest research trends in ncRNA \\
    \item LLM application in bioinformatics studies \\
    Advantages of LLM in bioinformatics studies. Especially, LLM can better resolve the challenges of ncRNA analysis than traditional comparative methods. \\
    Latest research trends in biological studies. \\
    \item List any previous studies on how data selection and quality influence model performance. 
\end{itemize}
\end{comment}


The study of non-coding RNA (ncRNA) attracts great attention in recent years due to its critical roles in multiple cellular processes, such as gene regulation, cellular differentiation, and development. However, the analysis of ncRNAs are challenging due to their diverse functions, complex gene regulatory mechanisms, and low expression levels compared to coding genes. 

Recent revolutional developments in artificial intelligence, particularly in natural language processing (NLP) has shine lights on genomic research. Large language models (LLMs) like GPT-3 have shown its remarkable ability on capturing complex dependencies and patterns in sequential data, and achieve great success in understanding and generating human languages. The application of LLMs are now emerging in biological sequence analysis.

Compared with coding genes, ncRNAs often lack clear sequence motifs or structural signatures, making their identification and functional prediction challenging. LLMs with ability to learn contextual information and long-range dependencies, could potentially overcome these limitations and provide new insights into ncRNA biology. Recent models like DNABERT, Nucleotide Transformer, and scGPT show state-of-the-art performance in various tasks, such as promoter-enhancer interaction prediction, functional elements identification in genomic sequences. 

In this study, we explore the potential and limitations of LLMs in ncRNA analysis by fine-tuning pre-trained foundation models. We focus on following tasks, including promoter region detection, coding and non-coding gene promoters classification, and prediction of gene expression levels. We aim to: \\
1. Evaluate the performance of state-of-the-art genomic language models (DNABERT, DNABERT-2, and Nucleotide Transformer) on ncRNA-related tasks.\\
2. Compare the LLMs with traditional machine learning methods, for example, logistic regression with n-gram TF-IDF features.\\
3. Investigate how data quality and selection influence model performance in the ncRNA-related tasks.\\
4. Gain biological insights into the regulatory mechanisms of ncRNAs through these analysis. \\

We designed a series of classification tasks that progressively increase the complexity and relevance to ncRNA analysis, including biological and artificial sequence classification, promoters sequence detection, coding and non-coding gene classification, and high and low expression genes classification. 
We also explore the interpretability of these models, attempting to extract biologically meaningful insights from their predictions. This aspect is particularly important in the field of ncRNA research to understand the functional elements and regulatory mechanisms.

By systematically evaluating the performance of LLMs on these ncRNA-related tasks, we hope to contribute to the development of more reliable computational methods for ncRNA research. 
This study not only evaluate the application of LLMs in ncRNA analysis but also aims to bridge the gap between computational predictions and biological understanding. 




==> section/method.tex <==

\section{Method}
\label{sec:method}

% \xr{describe how we propose to explore LLMs for non-coding RNA analysis here}

To explore the capability and limitations of pre-trained large-language models (LLMs) in non-coding RNA sequence analysis, we fine-tune pre-trained foundation models on multiple datasets.  
We mainly focus on the promoter sequences, which are important regions in the human genome that regulate gene expression. The ability of contextual information capture of LLMs may benefit the identification of functional elements and regulatory mechanisms to improve ncRNA analysis. 
These tasks are designed to provide insights into different aspects of ncRNA regulation and function. 

The biological and artificial sequence classification is not directly related to ncRNA analysis. This task serves as a critical quality check for the models. 
The promorer and non-promoter sequence classification task is designed to provide insights into the regulatory mechanisms of the promoter regions. Regulation of non-coding genes is often differs from the coding genes. 
The coding and non-coding gene promoter classification task is used to directly identifying the promoter regions of ncRNA genes. This taks can help us identify features that contribute to ncRNA regulation.
High and low expression gene promoter classification task is desinged to understand the features that associate with expression levels, which serves as a proxy to understand the regulatory difference between coding genes and non-coding genes. 

\subsection{Data}
We used three datasets for the LLM fine-tune, biological and artificial sequence dataset; promoter and non-promoter sequence dataset; promoter sequences of coding and non coding genes.

\textbf{The biological and artificial sequence dataset} is obtained from the GUE dataset\cite{zhou2023dnabert2}, the non-TATA promoter detection (human) dataset. This dataset includes 26533 positive samples and 26533 negative samples. Positive sequences are extracted from non-TATA promoter sequences, promoter sequences without TATA mofit, downloaded from the Eukaryotic Promoter Database (EPDnew)\cite{dreos2013epd}. Promoter sequences are extracted from the region 249bp before the transcription start site (TSS) and 50bp after. 
Negative samples are generated by random reshuffle of the positive sequences. Though the original study claimed that negative samples represents non-promoter sequences, the reshuffle of the biological sequences reduces the sequences to non-biological sequences, which is artificial sequences. Thus, in this study, we used this dataset for classification of biological and artificial sequences. The experiment shows that this task is easier compared to the real promoter classification task. 

\textbf{Promoter and non-promoter sequence dataset} is generated based on the non-TATA promoter sequence classification. We reused the positive samples from the GUE dataset. We regenerate negative samples by randomly sample 300bp sequences from the human genome with no overlap with any promoter region. Negative samples are biological sequences, but not promoter sequences, which align the task with the correct definition. This custom dataset contains 26533 positive samples from non-TATA data promoter detection dataset of GEU and 26533 negative samples. 


\textbf{Promoter sequence of coding and non-coding genes dataset} is another custom dataset we generated to further explore the limitation of the fine-tuned LLMs. We downlowd the human reference genome annotation file Homo\_sapiens.GRCh38.110.gtf from the Ensembl database. We extract the position of coding and non-coding genes by filtering the biotype of genes. 
The promoter sequences are extracted in the same way as those from Eukaryotic Promoter Database (EPDnew)~\cite{dreos2013epd}, where 300bp promoter sequence was extracted from the region of 249bp upstream of the transcription start site (TSS) and 50bp downstream from the human reference genome. 
This dataset contains 10239 positive samples and the same size of negative samples.

\textbf{Promoter sequence of high and low expression genes dataset} is constructed by following steps. The gene expression data of 49 tissues is downloaded from the Genotype-Tissue Expression (GTEx) V8 database. High expression genes are defined as gene expression over 75 percentile in all 49 tissues, and low expression genes are defined as gene expression below 25 percentile in all tissues. We generate promoter sequence dataset with different length $l$, 300bp, 500bp, 1000bp and 2000bp. All promoter sequences are extracted from the region of $l-50$ bp upstream of the TSS and 50 bp downstream.
Each dataset contains 2772 positive samples and 2772 negative samples.

\begin{table}[h]
    \centering
    \caption{Mean and standard deviation of gene expression for Coding and Non-coding genes.}
    \begin{tabular}{lcc}
        \hline
        & Mean & std \\
        \hline
        Coding gene & 44.93 & 792.96 \\
        Non coding gene & 0.94 & 6.63 \\
        \hline
    \end{tabular}
    \label{tab:gene_stats}
\end{table}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.7\textwidth]{figures/whole_blood.png}
  \vspace{-0.1in}
  \caption{Expression level statistics of coding (blue) and non-coding (red) genes.}
  \label{fig:gene_expression}
\end{figure}



\subsection{Foundation model fine-tuning}


%\xr{we can first provide some background about foundation models and why we choose to fine-tune them}
Foundation models (FMs) are language models pre-trained on large-scale dataset. These models are trained on a large amount of unlabeled data, which enable the models to learn general representations of biological sequences and capture complex dependencies and patterns. 

Fine-tuning the foundation models allows us to adapt these models to specific tasks, such as ncRNA sequence analysis, with limited computational resources. Prior studies have shown that fine-tuning foundation models in specific tasks can also significantly improve performance.

We fine-tune three state-of-the-art genome foundation models, DNABERT~\cite{ji2021dnabert}, DNABERT-2~\cite{zhou2023dnabert2} and Nucleotide Transformer~\cite{dalla2023nucleotide} on the proposed tasks to validate the impact of data quality on model performance, and gain biological insights into gene expression related regions in promoter sequences. Our approach to fine-tuning varies depending on the model architecture and computational constraints.

\textbf{DNABERT} is BERT-based foundation model for genome sequences analysis, which adapts the powerful contextual understanding capabilities. DNABERT is trained on overlapped k-mers (3/4/5/6) tokens derived from input DNA sequences. There are four variants of DNABERT model, DNABERT (3-mer), DNABERT (4-mer), DNABERT (5-mer), and DNABERT (6-mer), depending on the length of their tokenization. 

% \noindent
\textbf{DNABERT-2} is a refined genome foundation model derived from DNABERT with serveral improvements to expend its scalablity and reduce the cost of computational resource. Compared with DNABERT, DNABERT-2 adapts a more efficient tokenizer, utlizes multiple strategies to relax the constrains of inout sequence length, and pre-trained on multi-species genome with more sophisticated pre-training techniques to save computational resources. This helped the DNABERT-2 to achieve better generalization ability and delivers comparable performance with the state-of-the-art models. 

\textbf{Nucleotide Transformer (NT)} is a foundation model with an expanded scale of data and model parameters. There are four base NT models with 500M to 2.5B model parameters pre-trained on datasets of increasing size. The smallest model was not that small with 500M parameters trained on the Human reference genome. The largest base model with 2.5B parameters was trained on genome of 850 species. which provides exceptionally strong generalization power on downstream tasks. Due to capacity limitation, we selected the NT-500m-human, which is the 500M-parameter model pre-trained on human reference genome, and conducted a performance parameter efficient fine-tuning (PEFT) using Low-Rank Adaptation (LoRA)~\cite{hu2021lora}. 

For the fine-tuning of DNABERT and DNABERT-2, we perform a standard fine-tuning with AdamW~\cite{loshchilov2017decoupled} as optimizer. The learning rate is set to 3e-5, the batch size is set to 32, warmup step is 50, and the weight decay is 0.01. 
Since NT is one magnitude larger than the DNABERT and DNABERT-2 models, we performed fine-tuning using the LoRA technique to improve fune-tuning efficiency. The LoRA alpha is set to 16, dropout is 0.05, and r is 8. The learning rate is set to 1e-4. The parameters are reusing from DNABERT-2 based on a preliminary analysis of grid search on hyperparameter selections. All tasks share the same fine-tuning parameters. 

We use the Mathews correlation coefficient (MCC) to measure the model performance on three tasks. We also measured accuracy and F1-score on parameter sensitivity study on DNABERT with different k-mer for more comprehensive evaluation. 

\subsection{Simple model baseline}
To establish a benchmark performance, validate the necessity of using complex models and quantify the incremental value brought by advanced models, we set up a simple baseline using Logistic Regression (LR)\cite{cox1958regression} with n-gram Term Frequency-Inverse Document Frequency (TF-IDF)\cite{sparck1972statistical} features for three biological sequence classification tasks. LR is a widely used statistical method for binary classification tasks. In combination with n-gram TF-IDF features, LR becomes a powerful tool for sequence classification. Compared to large-scale foundation models, logistic regression requires minimal computational resources and is much faster to train and evaluate. 

% \xr{do we have some references for these simple baselines?}

We used biological and artifical sequence dataset, promoter and non-promoter sequence dataset, and promoter sequence dataset of coding and non-coding genes for model training and evaluation to have a fair comparison with advanced models. 

The sequences are segmented into n-grams, where the parameter $n$ ranges from 2 to 5. Then these n-grams are transformed into numerical representation using the TF-IDF method, which assigns weights to the n-grams based on their frequency in the individual sequence relative to their frequency in the entire dataset. A sparse matrix of TF-IDF features is used as input of logistic regression model.

\subsection{Feature importance analysis}

To gain deeper insight into which region contributes the most to the prediction of the model of the promoter sequence classification tasks, we performed a feature importance analysis based on the attention scores of the LLMs. The attention scores are aggregated and visualized to highlight the regions with the highest importance, which potentially associate to functional motifs that regulate gene expression.
To further prove the biological insights provided by LLMs, we can validate the findings by following approaches: (1) compare the identified important regions from the feature importance analysis with known regulatory motifs and elements from existing databases and publications; and (2) experimental validation by introduce modified promoter sequences with the predicted functional motifs into cellular models to evaluate its impact on gene expression. 

==> section/relate.tex <==
\section{Related Work}
\label{sec:relate}

The landscape of natural language processing has been transformed by the development of large language model (LLMs), which began with the Transformer architecture. LLMs, such as GPT-3~\cite{brown2020language}, are introduced based on the efficient attention mechanism to process sequential data. These models can capture complex dependencies in text, which makes them outperform traditional methods and applicable for biological sequence analysis. 

LLMs have significantly contributed to biological sequence analysis, such as DNA and RNA analysis, protein analysis, single-cell RNA sequence analysis, and non-coding RNA analysis. DNABERT~\cite{ji2021dnabert} and DNABERT-2~\cite{zhou2023dnabert2} are two advanced foundation models that trained for DNA analysis, and shows state-of-the-art performance in tasks such as promoter-enhancer interaction prediction. The Nucleotide Transformer~\cite{dalla2023nucleotide} extends to both DNA and RNA sequences.
Except for transformer-based models, Enformer~\cite{avsec2021effective} introduces a new architecture to predict gene expression from DNA sequences. HyenaDNA~\cite{nguyen2024hyenadna} combined aspects of transformers and long convolutions to model long-range dependencies in genomic sequences.
For protein sequence analysis and single cell RNA sequence analysis, LLMs also shows a significant contribution. The ESM-2 model~\cite{lin2023evolutionary} achieves state-of-the-art performance in protein structure and function prediction tasks. scGPT~\cite{cui2024scgpt} is built for scRNA sequencing data, and provides new insights cellular heterogeneity and gene expression patterns. 

Non-coding RNA (ncRNA) analysis is also benefit from LLM developments. Early work by Aoki introduced CNN for ncRNA classification \cite{aoki2018convolutional}. Recently, RNABERT \cite{akiyama2022informative}, introduced by Akiyama et al, showing significant improvement on ncRNA clustering and RNA structural alignment. 

LLMs become a efficient tools for biological sequence analysis. However, the impact of data quality on LLM performance was not fully understood. The data quality for model training and fine-tuning can significantly affect the model’s performance, potentially lead to wrong biological insights. In this paper, we will thoroughly discuss about how does the data quality influence the model performance. 



